On Tackling Complex Tasks with Reward Machines and Signal Temporal Logics

We propose a Reinforcement Learning (RL) based control design framework for handling complex tasks. The approach extends the concept of Reward Machines (RM) with Signal Temporal Logic (STL) formulas that can be used for event generation. The use of STL allows not only a more efficient representation of rewards for complex tasks but also guiding the training process to converge towards behaviors satisfying specified requirements. We also propose an implementation of the framework that leverages the STL online monitoring algorithms. We illustrate the framework with three case studies (minigrid, cart-pole and high-way environments) with non-trivial tasks.

==> algo.tex <==
\begin{figure}[htbp]\label{twoalgos}
%%\begin{minipage}{0.48\textwidth}
\begin{comment}
\begin{algorithm}[H]
\caption{Using a q-function $\hatQfct_v$ for each RM state $v_i$ of each RM $\RM_i$}\label{alg:QLearningRM}
    \begin{algorithmic}[1]
    
        \STATE $s = EnvInitState()$
        \STATE $u = SelectedRMInitState()$
        \STATE
        \FOR{$t \in \{1, \ldots, \timeHorizon\}$} 
        
            \IF{$\text{Terminal}(s)$}
                \STATE Break
            \ELSE
              \STATE $a = GetAct(\hatQfct_u, s)$
              \STATE $s' = EnvStep(s, a)$
              \STATE
              \STATE
              \STATE
              \STATE
             \STATE 
              \FOR{$v_i \in \mathbf{U}$}
                 \STATE $v_i' = \delta^i_u (v_i, L(s,a,s'))$
                 \STATE $r_i = \delta^i_r (v_i, v_i')$
                 \IF{$\text{Terminal}(s')$}
                   \STATE $\hatQfct_{v_i}(s, a) \leftarrow_{\alpha} r (s, a, s')$
                 \ELSE
                   \STATE $\hatQfct_{v_i}(s, a) \leftarrow_{\alpha} r (s, a, s')$
                   \STATE $\; \; \; + \gamma \max_{a'} \hatQfct_{v_i}(s', a')$
                 \ENDIF
             \ENDFOR  
            
        
            \STATE $u = \delta_u(u, L(s'))$, $s = s'$ \label{algo1updatestates}
            \ENDIF 
        \ENDWHILE
    \end{algorithmic}
\end{algorithm}
\end{comment}
%%\end{minipage}~~~~~
%%\begin{minipage}{0.48\textwidth}
\begin{algorithm}[H]
\caption{Using a q-function $\tildeQfct_i$ for each RM $\RM_i$ on the augmented states}\label{alg:QLearningRMaug}
    \begin{algorithmic}[1]
        \STATE $s = EnvInitState()$ 
        \STATE $\vu = RMInitStateVector()$
        \STATE $\vs = (s, \vu)$, $\traj = s$ 
        \FOR{$t \in \{1, \ldots, \timeHorizon\}$} 
            \IF{$\text{Terminal}(s)$}
                \STATE Break
            \ELSE
              \STATE $a = GetAct(\hatQfct_1, \ldots, \hatQfct_m, \vs)$
              \STATE $s' = EnvStep(s, a)$
              \STATE $\traj = Concat(\traj,s')$\label{lineConcat}
              
              
                \FOR{$j \in \{ 1, \ldots, m \}$}
                 \STATE $u_j' \leftarrow \delta^j_u (u_j, L(\traj))$ \label{lineUpdateRMstate}
               \ENDFOR
               \STATE $\vu' = ($u_1', \ldots, u_m')$ 
               \STATE $\vs' = (s', \vu')$ 
               \FOR{$j \in \{ 1, \ldots, m \}$}
                 \STATE $r_j = \delta^j_r (u_j, u_j')$
                 \IF{$\text{Terminal}(s')$}
                   \STATE $\tildeQfct_j(\vs, a) \leftarrow_{\alpha} r_j (s, a, s')$
                 \ELSE
                   \STATE $\tildeQfct_j(\vs, a) \leftarrow_{\alpha} r_j (s, a, s')$
                   \STATE $\; \; \; + \gamma \max_{a'} \tildeQfct_j(\vs', a')$
                 \ENDIF
             \ENDFOR 
            
             \STATE $\vu = \vu'$, $s = s'$
            
            \ENDIF  
        \ENDFOR
    \end{algorithmic}
\end{algorithm}
%%\end{minipage}

\caption{Algorithm~\ref{alg:QLearningRM} is one episode of QRM~\cite{Icarte2020}, Algorithm~\ref{alg:QLearningRMaug}} is one episode of our algorithm using augmented states and STL robustness in propositions.}
\end{figure}


==> algoPPO.tex <==
% \begin{algorithm}[tb]
% \caption{Using a q-function $\hat{q}_v$ for each RM state $v_i$ of each $RM_i$}
% \label{alg:QLearningRM}
% \begin{algorithmic}[1] %[1] enables line numbers
% \STATE $s = EnvInitState()$ \\
% \STATE $u = SelectedRMInitState()$\\
% \FOR{$t \in \{1, \ldots, T\}$} 
%     \IF{$\text{Terminal}(s)$}
%         \STATE Break
%     \ELSE
%         \STATE $a = GetAct(\hat{q}_u, s)$
%         \STATE $s' = EnvStep(s, a)$
%         \STATE 
%         \FOR{$v_i \in \mathbf{U}$}
%             \STATE $v_i' = \delta^i_u (v_i, L(s,a,s'))$
%             \STATE $r_i = \delta^i_r (v_i, v_i')$
%             \IF{$\text{Terminal}(s')$}
%                 \STATE $\hat{q}_{v_i}(s, a) \leftarrow_{\alpha} r (s, a, s')$
%             \ELSE
%                 \STATE $\hat{q}_{v_i}(s, a) \leftarrow_{\alpha} r (s, a, s')$
%                 \STATE $\; \; \; + \gamma \max_{a'} \hat{q}_{v_i}(s', a')$
%             \ENDIF
%         \ENDFOR  
%         \STATE $u = \delta_u(u, L(s'))$, $s = s'$ \label{algo1updatestates}
%     \ENDIF 
% \ENDFOR  
% \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}[tb]
% \caption{Using a q-function $\hat{q}_i$ for each $RM_i$ on the augmented states}
% \label{alg:QLearningRMaug}
% \begin{algorithmic}[1] %[1] enables line numbers
% \STATE $s = EnvInitState()$ 
% \STATE $\textbf{u} = RMInitStateVector()$
% \STATE $\textbf{s} = (s, \textbf{u}), w = s$ 
% \FOR{$t \in \{1, \ldots, T\}$} 
%     \IF{$\text{Terminal}(s)$}
%         \STATE Break
%     \ELSE
%         \STATE $a = GetAct(\hat{q}_1, \ldots, \hat{q}_m, \textbf{s})$
%         \STATE $s' = EnvStep(s, a)$
%         \STATE $w = Concat(w,s')$\label{lineConcat}
%         \FOR{$j \in \{ 1, \ldots, m \}$}
%             \STATE $u_j' \leftarrow \delta^j_u (u_j, L(w))$ \label{lineUpdateRMstate}
%         \ENDFOR
%         \STATE $\textbf{u}' = (u_1', \ldots, u_m')$ 
%         \STATE $\textbf{s}' = (s', \textbf{u}')$ 
%         \FOR{$j \in \{ 1, \ldots, m \}$}
%             \STATE $r_j = \delta^j_r (u_j, u_j')$
%             \IF{$\text{Terminal}(s')$}
%                 \STATE $\hat{q}_j(\textbf{s}, a) \leftarrow_{\alpha} r_j (s, a, s')$
%             \ELSE
%                 \STATE $\hat{q}_j(\textbf{s}, a) \leftarrow_{\alpha} r_j (s, a, s')$
%                 \STATE $\; \; \; + \gamma \max_{a'} \hat{q}_j(\textbf{s}', a')$
%             \ENDIF
%         \ENDFOR
%         \STATE $\textbf{u} = \textbf{u}'$, $s = s'$
%     \ENDIF  
% \ENDFOR
% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}[tb]

\caption{Proximal Policy Optimization (PPO) Algorithm}
\label{alg:PPO}
\begin{algorithmic}[1]
\STATE \textbf{Input:} Policy $\pi_\theta$, Value function $V_\phi$, Clip ranges $\epsilon$, $\epsilon_{vf}$, Coefficients $c_1$, $c_2$
    \WHILE{not converged}
    \STATE Initialize rollout buffer
    \FOR{$t = 1$ to $n_{\text{steps}}$}
        \STATE Sample action $a_t \sim \pi_\theta(a_t | s_t)$
        \STATE Execute $a_t$ in environment to get $r_t$, $s_{t+1}$
        \STATE Store $(s_t, a_t, r_t, \log \pi_\theta(a_t|s_t), V_\phi(s_t))$
    \ENDFOR
    \STATE Compute advantages $A_t$ using GAE
    \STATE Compute returns $R_t = A_t + V_\phi(s_t)$

    \FOR{$k = 1$ to $n_{\text{epochs}}$}
        \FOR{each minibatch from rollout buffer}
            \STATE Compute $\pi_\theta(a|s)$, $V_\phi(s)$, entropy $H(\pi_\theta)$
            \STATE Compute probability ratio: $r(\theta) = \frac{\pi_\theta(a|s)}{\pi_{\theta_{\text{old}}}(a|s)}$
            \STATE Compute clipped surrogate loss:
            \[
                L^{\text{CLIP}} = \mathbb{E}\left[\min(r(\theta)A, \text{clip}(r(\theta), 1 - \epsilon, 1 + \epsilon)A)\right]
            \]
            \STATE Compute value loss:
            \[
                L^{VF} = \begin{cases}
                    \text{MSE}(R, \text{clip}(V_\phi, V_{\text{old}} - \epsilon_{vf}, V_{\text{old}} + \epsilon_{vf})) &  \\\text{if clipping} \\
                    \text{MSE}(R, V_\phi) & \\ \text{otherwise}
                \end{cases}
            \]
            \STATE Compute total loss:
            \[
                L = -L^{\text{CLIP}} + c_1 \cdot L^{VF} - c_2 \cdot H(\pi_\theta)
            \]
            \STATE Update $\theta, \phi$ using gradient descent (with gradient clipping)
        \ENDFOR
    \ENDFOR
\ENDWHILE
\end{algorithmic}
\end{algorithm}

% \caption{Algorithm~\ref{alg:QLearningRM} is one episode of QRM~\cite{Icarte2020}, Algorithm~\ref{alg:QLearningRMaug}} is one episode of our algorithm using augmented states and STL robustness in propositions.}
% \end{figure}

\begin{algorithm}[H]
\caption{PPO Training with Reward Machine-Augmented Observations}
\label{alg:PPORM}
\begin{algorithmic}[1]
\STATE \textbf{Input:} Gymnasium environment $env$, reward machine $RM$, PPO agent $\pi_\theta$, value function $V_\phi$
\STATE \textbf{Initialize:} PPO policy $\theta$ and value $\phi$ parameters 
\FOR{each iteration}
    \STATE Initialize episode: $s \leftarrow env.reset()$, $u \leftarrow RM.reset()$
    \FOR{$t = 1$ to $T$}
        \STATE $obs \leftarrow \text{concat}(s, u)$ \COMMENT{Augment state with RM state}
        \STATE $a \sim \pi_\theta(\cdot | obs)$ \COMMENT{Sample action from current policy}
        \STATE Execute action $a$: observe $s'$, env reward $r_{\text{env}}$, done
        \STATE $r_{\text{rm}} \leftarrow RM.get\_reward(s, a, s')$ 
        \STATE $r \leftarrow r_{env} * r_{rm}$
        \STATE $u' \leftarrow RM.update(u, s, a, s')$ \COMMENT{Update RM state}
        \STATE $obs' \leftarrow \text{concat}(s', u')$
        \STATE Store transition $(obs, a, r, obs', \text{done})$
        \STATE $s \leftarrow s'$, $u \leftarrow u'$
        \IF{done or truncated} 
            \STATE Reset environment and RM
            \STATE $s \leftarrow env.reset()$, $u \leftarrow RM.reset()$
        \ENDIF
    \ENDFOR
    \STATE Compute $A_t$
    \STATE Update $\pi_\theta$ and $V_\phi$ 
\ENDFOR
\end{algorithmic}
\end{algorithm}
